VarAD: Lightweight High-Resolution Image Anomaly Detection via Visual Autoregressive Modeling

This paper addresses a practical task: High-Resolution Image Anomaly Detection (HRIAD). In comparison to conventional image anomaly detection for low-resolution images, HRIAD imposes a heavier computational burden and necessitates superior global information capture capacity. To tackle HRIAD, this paper translates image anomaly detection into visual token prediction and proposes VarAD based on visual autoregressive modeling for token prediction. Specifically, VarAD first extracts multi-hierarchy and multi-directional visual token sequences, and then employs an advanced model, Mamba, for visual autoregressive modeling and token prediction. During the prediction process, VarAD effectively exploits information from all preceding tokens to predict the target token. Finally, the discrepancies between predicted tokens and original tokens are utilized to score anomalies. Comprehensive experiments on four publicly available datasets and a real-world button inspection dataset demonstrate that the proposed VarAD achieves superior high-resolution image anomaly detection performance while maintaining lightweight, rendering VarAD a viable solution for HRIAD. Code is available at \href{https://github.com/caoyunkang/VarAD}{\url{https://github.com/caoyunkang/VarAD}}.

==> tables/Table_adapter.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[t]
% \centering
% \caption{Ablation study on the feature adapter of VarAD.}
% \label{tab:adapter}
% % \setlength\tabcolsep{15.0pt}
% \begin{tabular}{@{}ccc@{}}
% \toprule[1.5pt]
% Dataset  & w/ Adapter                & w/o Adapter                \\ \midrule
% MVTec AD~\cite{MVTec-AD} & (97.7, 63.8, 63.0) & (95.3, 50.1, 47.6) \\
% VisA~\cite{VisA}     & (98.5, 47.5, 40.7) & (97.9, 37.5, 31.1) \\
% BTAD~\cite{BTAD}     & (97.8, 63.6, 64.5) & (97.2, 54.4, 51.3) \\
% DTD-Synthetic~\cite{DTD}      & (98.8, 77.3, 80.9) & (97.3, 73.4, 75.9) \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table*}[t]
% \centering
% \caption{}
% \label{tab:adapter}
% \begin{tabular}{@{}ccccccc@{}}
% \toprule[1.5pt]
% Linear   Layer &
%   \ding{52} &
%   \ding{52} &
%   \textcolor{gray}{\ding{56}} &
%   \textcolor{gray}{\ding{56}} &
%   \ding{52} &
%   \textcolor{gray}{\ding{56}} \\
% ResBlock &
%   \textcolor{gray}{\ding{56}} &
%   \textcolor{gray}{\ding{56}} &
%   \ding{52} &
%   \textcolor{gray}{\ding{56}} &
%   \textcolor{gray}{\ding{56}} &
%   \ding{52} \\
% LoRA     & \textcolor{gray}{\ding{56}} & \textcolor{gray}{\ding{56}} & \textcolor{gray}{\ding{56}} & \ding{52}          & \ding{52}            & \ding{52}          \\ \midrule
% MVTec AD & (95.3, 50.1, 47.6)          & (97.7, 63.8, 63.0)          & (97.0, 58.4, 57.8)          & (95.1, 48.0, 44.4) & (97.5, 62.6, 62.3)   & (97.1, 59.3, 58.8) \\
% VisA     & (97.9, 37.5, 31.1)          & (98.5, 47.5,   40.7)        & (98.7, 47.5, 42.9)          & (97.3, 34.2, 27.5) & (98.3, 46.1, 39.5)   & (98.9, 48.9, 44.9) \\
% BTAD     & (97.2, 54.4, 51.3)          & (97.8, 63.6, 64.5)          & (97.7, 59.4, 60.4)          & (97.2, 53.1, 49.2) & (97.5, 62.1,   63.9) & (97.9, 60.8, 62.8) \\
% DTD      & (97.3, 73.4, 75.9)          & (98.8, 77.3, 80.9)          & (97.7, 76.1, 78.9)          & (97.4, 73.4, 75.8) & (98.7, 77.9, 81.6)   & (97.8, 75.7, 78.5) \\ \bottomrule[1.5pt]
% \end{tabular}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering

\caption{Ablation study on the feature adapter of VarAD. w/o indicates that the pre-trained model is used to directly extract tokens.}
\label{tab:adapter}
\setlength\tabcolsep{10.0pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule[1.5pt]
Dataset & w/o              & LoRA               & Linear Layer              & Linear Layer+LoRA          & ResBlock           & ResBlock+LoRA      \\ \midrule
MVTec AD~\cite{MVTec-AD} & (95.3, 50.1, 47.6) & (95.1, 48.0, 44.4) & (\textbf{97.7}, \textbf{63.8}, \textbf{63.0}) & (\underline{97.5}, \underline{62.6}, \underline{62.3}) & (97.0, 58.4, 57.8) & (97.1, 59.3, 58.8) \\
VisA~\cite{VisA}    & (97.9, 37.5, 31.1) & (97.3, 34.2, 27.5) & (98.5, \underline{47.5},   40.7) & (98.3, 46.1, 39.5)   & (\underline{98.7}, \underline{47.5}, \underline{42.9}) & (\textbf{98.9}, \textbf{48.9}, \textbf{44.9}) \\
BTAD~\cite{BTAD}    & (97.2, 54.4, 51.3) & (97.2, 53.1, 49.2) & (\underline{97.8}, \textbf{63.6}, \textbf{64.5})   & (97.5, \underline{62.1},   63.9) & (97.7, 59.4, 60.4) & (\textbf{97.9}, 60.8, \underline{62.8}) \\
DTD-Synthetic~\cite{DTD}     & (97.3, 73.4, 75.9) & (97.4, 73.4, 75.8) & (\textbf{98.8}, \underline{77.3}, \underline{80.9})   & (\underline{98.7}, \textbf{77.9}, \textbf{81.6})   & (97.7, 76.1, 78.9) & (97.8, 75.7, 78.5) \\ \bottomrule[1.5pt]
\end{tabular}
}

\end{table*}


==> tables/Table_hierarchy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\caption{Quantitative comparisons of VarAD under different feature hierarchies. 
% Results are presented as (AUROC\%, max-F1\%, AP\%). Best scores are highlighted in \textbf{bold}, while the second-best scores are also \underline{underlined}.
}
\label{tab:hierarchy}
% \setlength\tabcolsep{10.0pt}
\setlength\tabcolsep{10.0pt}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule[1.5pt]
Dataset & 4th                & 8th                & 12th               & 4th+8th            & 8th+12th           & 4th+8th+12th       \\ \midrule
MVTec AD~\cite{MVTec-AD}      & (94.0, 50.5, 47.4) & (97.0, 59.4, 58.7)   & (97.0, 59.9, 57.9) & (97.0, 60.7, 60.0) & (\underline{97.6}, \underline{63.5}, \underline{62.9}) & (\textbf{97.7}, \textbf{63.8}, \textbf{63.0})   \\
VisA~\cite{VisA}    & (94.9, 29.2, 22.6) & (98.1, 42.1, 34.4) & (\underline{98.4}, \textbf{47.9}, \textbf{41.1}) & (97.6, 43.0, 35.9) & (98.3, 46.9, 40.3) & (\textbf{98.5}, \underline{47.5}, \underline{40.7}) \\
BTAD~\cite{BTAD}    & (92.1, 36.2, 33.4) & (\textbf{97.9}, \underline{62.6}, 63.1) & (96.8, 58.6, 58.4) & (97.3, 60.8, 62.2) & (97.4, 62.6, \underline{64.3}) & (\underline{97.8}, \textbf{63.6}, \textbf{64.5}) \\
DTD-Synthetic~\cite{DTD} & (92.3, 62.9, 61.3) & (98.7, \underline{78.0},   81.6) & (98.4, 71.7, 73.4) & (98.4, \textbf{78.2}, \textbf{81.6}) & (\underline{98.7}, 78.0, \underline{81.6}) & (\textbf{98.8}, 77.3,   80.9) \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table*}

==> tables/Table_main_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\centering
\caption{Quantitative comparisons of VarAD with alternative methods on public datasets. Results are presented as (AUROC\%, max-F1\%, AP\%). Best scores are highlighted in \textbf{bold}, while the second-best scores are also \underline{underlined}.}
\label{tab:main_performance}
\resizebox{1.\linewidth}{!}{
\setlength\tabcolsep{10.0pt}
\begin{tabular}{@{}ccccccccc @{}}
\toprule[1.5pt]
Dataset &
  \begin{tabular}[c]{@{}c@{}}PFM~\cite{PFM}\\      TII'2022\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RD4AD~\cite{RD4AD}\\      CVPR'2022\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PatchCore~\cite{Patchcore}\\      CVPR'2022\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}CDO~\cite{CDO}\\      TII'2023\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PyramidFlow~\cite{PyramidFlow}\\      CVPR'2023\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AMI-Net~\cite{AMI-Net}\\      TASE'2024\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PNPT~\cite{PNPT}\\      TII'2024\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}VarAD\\      Proposed\end{tabular} \\ \midrule
MVTec AD~\cite{MVTec-AD} & (91.3, 36.6,   27.9) & (93.4, 49.6, 42.5) & (95.8, 60.1, 60.5) & (\underline{96.4}, \underline{62.8}, \underline{62.9}) & (94.2, 48.9, 43.4) &(94.9, 53.2, 49.9)& (94.8, 52.3, 50.8)& (\textbf{97.7}, \textbf{63.8}, \textbf{63.0})   \\
VisA~\cite{VisA}  & (94.6, 14.2, 06.7)   & (92.9, 39.0, 26.8) & (95.1, \underline{46.6}, {38.9}) & (\underline{97.6}, {46.5}, {37.7}) & (90.8, 32.4, 24.2) &(96.9, 38.6, 34.0)& (96.7, 45.0, \underline{40.3}) & (\textbf{98.5}, \textbf{47.5},   \textbf{40.7}) \\
BTAD~\cite{BTAD}  & (97.5, 54.7, 50.6)   & (97.6, 51.1, 50.0) & (97.0, 50.1, 47.5) & (\underline{97.7}, \underline{57.1}, \underline{56.5}) & (88.7, 37.8, 32.2) &(96.0, 50.2, 39.4) & (97.5, 54.4, 51.5) &  (\textbf{97.8}, \textbf{63.6}, \textbf{64.5})   \\
DTD-Synthetic~\cite{DTD}   & (91.8, 37.6, 29.2)   & (95.3, 45.1, 33.1) & (96.0, 70.6, 70.8) & (\underline{97.4}, \underline{72.3}, \underline{75.5}) & (96.6, 52.1, 43.3) & (94.4, 61.1, 60.9) & (93.7, 61.1, 59.3) & (\textbf{98.8}, \textbf{77.3}, \textbf{80.9})   \\ \bottomrule[1.5pt]
\end{tabular}
}

\end{table*}

==> tables/Table_path.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\caption{Quantitative comparisons of VarAD under different scanning directions. 
% Results are presented as (AUROC\%, max-F1\%, AP\%). Best scores are highlighted in \textbf{bold}, while the second-best scores are also \underline{underlined}.
}
\label{tab:path}
\resizebox{1\linewidth}{!}{
\setlength\tabcolsep{16.0pt}
\begin{tabular}{@{}cccccc@{}}
\toprule[1.5pt]
 Dataset    & k=1                & k=2                & k=3                & k=4                & All                \\ \midrule
MVTec AD~\cite{MVTec-AD}      & (97.0, 62.3, 61.2) & (97.4, \underline{62.8}, \underline{62.1}) & (\underline{97.5}, 62.5,   62.0) & (97.3, 62.1, 61.1) & (\textbf{97.7}, \textbf{63.8}, \textbf{63.0}) \\
VisA~\cite{VisA} & (98.4, 47.0, 40.2) & (98.4, 47.2, \underline{40.4}) & (98.3, 45.7, 39.1) & (\underline{98.4}, \underline{47.2}, 40.3) & (\textbf{98.5}, \textbf{47.5}, \textbf{40.7}) \\
BTAD~\cite{BTAD} & (97.6, 62.7, 63.8) & (97.7, 63.1, 64.3) & (97.7, 62.9, 64.2) & (\underline{97.8}, \underline{63.4}, \underline{64.4}) & (\textbf{97.8}, \textbf{63.6}, \textbf{64.5}) \\
DTD-Synthetic~\cite{DTD} & (98.8, 76.7, 80.2) & (98.8, 76.8, 80.2) & (\underline{98.8}, 76.5, 79.6) & (98.7, \underline{76.9}, \underline{80.3}) & (\textbf{98.8}, \textbf{77.3}, \textbf{80.9}) \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table*}
